"Actually I Can Count My Blessings": User-Centered Design of an Application to Promote Gratitude Among Young Adults

Regular practice of gratitude has the potential to enhance psychological wellbeing and foster stronger social connections among young adults. However, there is a lack of research investigating user needs and expectations regarding gratitude-promoting applications. To address this gap, we employed a user-centered design approach to develop a mobile application that facilitates gratitude practice. Our formative study involved 20 participants who utilized an existing application, providing insights into their preferences for organizing expressions of gratitude and the significance of prompts for reflection and mood labeling after working hours. Building on these findings, we conducted a deployment study with 26 participants using our custom-designed application, which confirmed the positive impact of structured options to guide gratitude practice and highlighted the advantages of passive engagement with the application during busy periods. Our study contributes to the field by identifying key design considerations for promoting gratitude among young adults.

==> First_Version/formative_results.tex <==
\section{Formative Study Findings}
Our formative work identified several themes related to the desirable features participants envisioned in gratitude-promoting applications. In the following sections, we will discuss each of these themes and their implications for our subsequent deployment study.
%\subsection{Ease of use}

%Majority of the participants 



\subsection{Desired Structure for Gratitude Practice}

%Some participants, who had previously used paper-based gratitude journals, reported that their positive experiences motivated them to use mobile application versions of the practice. One participant (P3) mentioned that they had used a paper-based gratitude journal before and found it helpful to think more positively and less negatively.
\todo{Focus more on examples and structures}
Some participants who had prior experience with paper-based gratitude journals expressed their motivation to transition to mobile application versions of the practice based on their past positive experiences. For instance, FP3 highlighted that using a paper-based gratitude journal had been beneficial in promoting more positive thinking and reducing negative thoughts.
FP13 stated, \textit{``I used to keep a gratitude journal ... I thought it was a brilliant way of trying to keep on the positive side of things ... and it helped with anxiety or even negative thinking.''} These firsthand experiences with paper-based gratitude journaling led to their continued use of mobile application versions of the practice.

However, not all participants had a similar level of experience with practicing gratitude, and those who were doing it for the first time found the activity more difficult. This sentiment was apparent in FP4's statement:

\italquote{If I’d had a better idea of stuff to put into it, maybe I would've used it more, but I didn’t really know what to put into it.}


Despite the initial challenges faced by some participants, they expressed that with consistent practice, they were able to develop an increased ability to identify and appreciate things they were grateful for. They emphasized the importance of additional support from the application, such as more information or clear instructions, to aid them in overcoming the initial hurdles in their gratitude practice. Even participants with prior experience in practicing gratitude, like P14, echoed this need for guided support. P14 mentioned that such features could aid in recalling and appreciating grateful moments or events that might otherwise be overlooked during the day.



%This need for support was echoed by more experienced participants with gratitude too, as P14 expressed that they might forget about the grateful moments or events on a day and in those cases, some hints or structure would enable them to remember and cherish them.

%This suggests that the practice of gratitude journaling may initially require effort and persistence, but over time, it could become more accessible and rewarding as individuals develop a heightened awareness of positive aspects of their lives.
%Participants, however, informed us that with regular practice, they discovered that they were able to think of more things to be grateful for. This indicates that the practice of gratitude journaling may require some effort and persistence, but with time, it can become more accessible and beneficial.
%Participants also opted for a simple design and 

\noindent
\textbf{Implications for Our Deployment:} %The diverse range of skill levels observed among people when it comes to practicing gratitude served as the primary motivation for our experimentation with two design ideas. 

\revision{Previous research has highlighted the effectiveness of providing examples and instructions to individuals, helping them to better understand and adopt a psychological principle in their life \cite{bhattacharjee2022kind, o2018suddenly}.  This insight emerged as particularly relevant in our formative study, where participants indicated that structured guidance could greatly enhance their experience with gratitude-promoting applications. Such guidance, which includes clear instructions and relevant examples, can be especially beneficial for both novices and seasoned practitioners of gratitude exercises. It might offer a sense of direction, mitigating the initial overwhelm associated with starting a new habit and helping to establish a foundation for regular engagement with the tool \cite{bhattacharjee4057942exploring}. However, many existing applications, including those used in our formative study, opt for a more open-ended approach to support journaling. This flexibility might cater to users who might find structured methods constraining and prefer a less guided experience \cite{furnham2011literature}. To delve deeper into the benefits and potential drawbacks of structured guidance in gratitude journaling, our deployment study participants were divided into two groups:}

\begin{itemize}
    \item \textbf{Experiment Group:} Participants were provided with options to select life areas they were feeling grateful for, \revision{accompanied by explanations and examples}, before making daily gratitude entries in the application. 
    \item \textbf{Control Group:} Participants were asked to make daily gratitude entries in the application without any options to select life areas.
\end{itemize}

%However, there is a potential risk associated with such guidance, as it may limit people's thoughts and restrict the range of potential life areas for which they can feel grateful \cite{furnham2011literature}.
%This allowed us to investigate the effectiveness of each approach and determine which method was most effective in promoting gratitude among participants with varying skill levels.

\subsection{Role of Timing and Social Contexts}

Participants highlighted the importance of having suitable contexts that provided them with the necessary time and space to engage with the gratitude applications.  They reported using the gratitude applications most often when alone, affording time for reflection; ``\textit{You have to focus on it, and if around people, I would have rushed it.}'' (FP17). Some participants expressed that being around other people could hinder the state of mind required for practicing gratitude. FP14, for instance, remarked that doing it at a table while in the company of others did not feel like the right time to practice gratitude.  As a result, participants tended to use the applications after regular working hours,  specifically in the evening before going to bed. This time frame provided them with the opportunity to engage in reflection without distractions, ensuring sufficient time and privacy for their gratitude practice. %For example,  P17 mentioned that they found it helpful to stay up late at night when everyone else had gone to bed, so that they could reflect on their day and write about the things they were grateful for. 
FP17 saw this as a form of ``me time'' that allowed for more focused reflection. Participants also indicated the need for a routine to positively influence the use of the application. FP13 suggested that doing the activity at a particular time everyday had made it easier for them to keep up and eventually recognize the benefits of gratitude. 

Lastly, participants expressed a preference for privacy while using the gratitude journaling application, as it was considered a personal and introspective activity. To ensure this privacy, they suggested an incognito darker color scheme for the application interface so that the mobile screen is not easily visible to people around.

\noindent
\textbf{Implications for Our Deployment:}
%In the evening, people often find themselves alone and with some free time after a long day of work. This can be a great opportunity for them to reflect on the positive elements in their life and cultivate feelings of gratitude. Research has shown that practicing gratitude regularly can lead to numerous physical and mental health benefits, including improved sleep, reduced stress, and increased happiness.
Prior research works \cite{bhattacharjee2022design, bhattacharjee2023investigating, park2015manifestation} show that young adults generally prefer afternoons and evenings  for reflecting on positive aspects of life since they generally have more free time then and are not in a rush to get to work or school like in the morning. Our formative study participants also shared similar opinions.
Therefore, our prototype application used in the deployment study sent notifications at 6 pm everyday. This time was chosen as it is a period when people are more likely to have some free time after working hours, but not too late that they may be too tired. 

\revision{The decision to send notifications at a fixed time, as opposed to randomizing them within an evening window, was grounded in the principles of habit formation and behavioral consistency. Research in behavioral psychology suggests that consistent cues, such as a notification at the same time every day, can significantly enhance habit formation \cite{eyal2014hooked, stawarz2014don}. Furthermore, \citet{lally2010habits}'s work on habit formation emphasizes the role of consistency in cue-response routines in establishing new habits. By aligning the notification timing with the natural downtime of our target demographic and reinforcing a consistent daily routine, we, therefore, aimed to embed the gratitude practice more effectively into participants' daily lives to support sustained engagement and habit formation.}

%By sending notifications consistently at the same time each day, we also wanted to help participants establish a habit of practicing gratitude \cite{eyal2014hooked, stawarz2014don}.

Additionally, participants emphasized the importance of privacy while using the application, in line with previous research \cite{eamons2003counting, o2017design}. We incorporated their feedback by using a dark blue background for the application interface.


% \subsection{Hesitancy in sharing gratitude entries on social media platforms}

% The social media sharing functionality within the applications allows users to share a post related to the exercise across social media channels. None of the participants reported using this functionality, with many describing social media as an inappropriate platform from which to elicit support, referencing the private nature of the exercise. Participants suggested that the awareness that others would be reading and judging what they wrote had the potential to interfere with the exercise. For example, P1 said, 

% \italquote{I found the idea that I would share [the entry] was counter to the whole point ... because then it becomes an image construction thing instead of something helpful for you, so I just didn’t engage with that.}  

% This suggests that privacy can be an important factor in practicing gratitude and that people may prefer to use the application in private settings where they feel more comfortable sharing their thoughts and feelings.

% \textbf{Implications for our deployment:}

% private and no media sharing

\subsection{Benefits of Labeling Mood}

The majority of the participants expressed that their  emotional states, both before and after practicing gratitude, would influence their motivation to use the application. Most participants reported experiencing a positive shift in mood as a result of logging an entry, even when their initial mood was negative. FP15 said,

\italquote{It kind of shifted me if I was having a bad day. Made me kind of, well actually, I am going to focus here on the good things. ... There was a very conscious shift in my thinking on the bad days. I became more aware of trying to focus on the positives.}

Participants indicated that engaging in regular mood labeling and reviewing them at a later time would facilitate their ability to recognize negative thought patterns and triggers that influence their thoughts and emotions. This heightened awareness would, in turn, make them more receptive to the practice of gratitude as they actively sought out positive aspects of their lives to document and reflect on. Additionally, seeing improvements in their mood when they focused on positive experiences also served as reinforcement, further encouraging individuals to continue practicing gratitude.  

\noindent
\textbf{Implications for Our Deployment:} Our formative study findings led us to incorporate brief mood labeling questions before and after the gratitude activity in our application. Previous research has highlighted the benefits of mood labeling, such as increased awareness of emotions and thought patterns, which contributes to a better understanding of one's mental states \cite{torre2018putting,  huang2015emotion, kou2020emotion}. Therefore, we included a single question asking participants to rate their mood on a scale of 1 to 5 (1 = very low mood, 3 = neutral, 5 = very high mood) before and after engaging in the gratitude activity. This approach had the potential to capture participants' mood changes while minimizing the burden of extensive questioning \cite{bhattacharjee2023investigating}.





%However, participants in our study expressed a preference for concise questions. 

%Our formative study findings motivated us to ask users brief emotion-labeling questions before and after the gratitude activity. Prior research has also noted several benefits of emotion labeling \cite{torre2018putting, bhattacharjee2023investigating}; for example, labeling emotions can help individuals become more aware of their emotions and thought patterns, facilitating a better understanding of their own mental states \cite{bhattacharjee2023investigating}. However, our participants expressed that those questions should be brief, so we asked only one question that asked them to rate their mood on a 1 to 5 scale (1 = very low mood to 3 = neutral to 5 = very high mood) before and after the activity.


%\subsection{Design of Interface}


==> Scrap/quant.tex <==
We conducted a linear regression analysis to examine the relationship between word count ($WordCount$) and the predictor variables, including the initial mood entry ($moodBefore$) and group (control vs. experiment). The model equation was as follows: $WordCount = \beta0 + \beta1 * MoodBefore + \beta2 * Group$.

\begin{table}[]
    \caption{\todo{Caption --- What was baseline}}
    \label{tab:regression}
    \centering
    \begin{tabular}{cccc}\\\hline
         & Estimate & Standard Error & p-value  \\\hline
         (Intercept) & 7.99 & 4.34 & 0.07\\\hline
         $MoodBefore$ & 0.28 & 1.25 & 0.82\\
         $Group (Experiment)$ & 6.38 & 2.04 & 0.002**\\\hline
         \multicolumn{4}{l}{\footnotesize{* p-value \textless 0.05, ** p-value \textless 0.01}}
    \end{tabular}

\end{table}

The result of the regression analysis is presented in Table \ref{tab:regression}. The findings indicate a significant difference in word count between the experiment and control groups (p = 0.002), suggesting that the presence of life area options in the experiment group positively influenced active engagement. The overall regression model was statistically significant too ($F(2, 172) = 4.88, p < 0.001$).
This result provides promising evidence for the benefits of life area options; however, it is crucial to consider that other factors might also contribute to the observed differences in engagement levels (the adjusted R-squared value for the regression model was found to be 0.04). For a more comprehensive understanding, qualitative data in Section \ref{subsubsec:life_area} provide additional support and insights into the relationship between the presence of life area options and active engagement.
